ESREAL: Exploiting Semantic Reconstruction to Mitigate Hallucinations in Vision-Language Models

Hallucinations in vision-language models pose a significant challenge to their reliability, particularly in the generation of long captions. Current methods fall short of accurately identifying and mitigating these hallucinations. To address this issue, we introduce ESREAL, a novel unsupervised learning framework designed to suppress the generation of hallucinations through accurate localization and penalization of hallucinated tokens. Initially, ESREAL creates a reconstructed image based on the generated caption and aligns its corresponding regions with those of the original image. This semantic reconstruction aids in identifying both the presence and type of token-level hallucinations within the generated caption. Subsequently, ESREAL computes token-level hallucination scores by assessing the semantic similarity of aligned regions based on the type of hallucination. Finally, ESREAL employs a proximal policy optimization algorithm, where it selectively penalizes hallucinated tokens according to their token-level hallucination scores. Our framework notably reduces hallucinations in LLaVA, InstructBLIP, and mPLUG-Owl2 by 32.81%, 27.08%, and 7.46% on the CHAIR metric. This improvement is achieved solely through signals derived from the image itself, without the need for any image-text pairs.

==> Algorithms/1_reward_calculation.tex <==
\begin{algorithm}[!h]
\footnotesize
\begin{algorithmic}[1]
\REQUIRE T2I: Text-to-Image Model, $G$: grounding model, CLIP: similarity model
\REQUIRE $\textrm{I}$: Input image, $s_{1..T}$: Generated caption from the image

\STATE Initialize $p_{{\textrm{H1}}, t}$ and $p_{{\textrm{H1}}, t}$ to 0 for $t = 1$ to $T$
% \FOR{${i=1}$ to $T$}
%     \STATE $p_{{H1}, t} = 0$ \hfill $\leftarrow$ Initialize penalty for H1
%     \STATE $p_{{H2}, t} = 0$ \hfill $\leftarrow$ Initialize penalty for H2
% \ENDFOR
\STATE $\textrm{I}_{rec} \leftarrow \textrm{T2I}(s_{1..T})$ % \hfill $\leftarrow$ Reconstruct image from text
\STATE $\{(s_{{b_j}..{e_j}}, \textrm{I}_{rec}^j)\}_{j=1}^N$ $\leftarrow$ $G(s_{1..T}, \textrm{I}_{rec})$  % \hfill $\leftarrow$ Grounding on reconstructed image and get object-region pairs
\STATE{Loop over object-region pairs in a batched manner:}
\FOR{${j=1}$ to $N$}
    \STATE $(s_{{b^\prime_j}..{e^\prime_j}}, \textrm{I}^j)$ $\leftarrow$ $G(\{s_{{b_j}..{e_j}}\}, \textrm{I})$ % \hfill $\leftarrow$ Grounding on original image
    \IF{$(s_{{b^\prime_j}..{e^\prime_j}}, \textrm{I}^j) = \emptyset$}
        \STATE $p_{\textrm{H1}, e_j} = -1$ \hfill $\leftarrow$ Penalty for non-existent objects
    \ELSE
        \STATE $p_{\textrm{H2}, e_j} = (1 - \textrm{CLIP}(\textrm{I}^j, \textrm{I}_{rec}^j))/2$ \hfill $\leftarrow$ Penalty for unfaithful object attributes
    \ENDIF
\ENDFOR
\STATE $p_{rec} = - \textrm{CLIP}(\textrm{I}, \textrm{I}_{rec})$ \hfill $\leftarrow$ Penalty for overall reconstruction

\caption{Reward Calculation}
\label{alg:reward_calculation}
\end{algorithmic}
\end{algorithm}

==> Algorithms/2_ppo_training.tex <==
\begin{algorithm}[!h]
% \footnotesize
\begin{algorithmic}[1]
% \State {\bfseries Input:} 
\REQUIRE policy $\pi_\theta$, reference policy $\pi_{\text{ref}}$, value model $V_\phi$, reward model $r$, PPO clipping parameter $\epsilon$, step size $\alpha$, number of epochs $E$, batch size ${B}$, image dataset $\mathcal{D}$, hallucination penalty weights $w_{H1}, w_{H2}, w_{H3}$, KLD scaling parameter $\beta$
% \State {\bfseries Output:} the trained policy $\pi_\theta$ % and value function $V_\phi$ 
\REPEAT
\STATE Sample batch $\{x^i\}_{i=1}^B \sim \mathcal{D}$ with batch size ${B}$
\STATE Sample output sequence $a^i_{1..T} \sim p_\theta(a_{1..T}|x^i, a_0)$ for each of the data $x^i$ in batch
\STATE Compute rewards $r^i_{1..T}$ using reward model $ r(x^i, a^i_{0..T})$ for each output sequence
\STATE Compute advantages $A^i_{1..T}$ using Generalized Advantage Estimation (GAE):
\STATE \quad $\delta^i_t = r^i_{t} + \gamma V_\phi(s^i_{t+1}) - V_\phi(s^i_t)$
\STATE \quad $A^i_t = \delta^i_t + (\gamma \lambda) \delta^i_{t+1} + \cdots + (\gamma \lambda)^{T-t+1} \delta^i_{T-1}$
\STATE Compute value targets $V^i_{t=1..T}$ with $V^i_t = \sum_{t^\prime=t}^T r^i_t$
\FOR{PPO epoch $i = 1, \dots, E$}
    % \STATE Update policy $\pi_\theta$ and value function $V_\phi$ using the PPO objective:
    \STATE Update policy $\pi_\theta$ using the clipped surrogate objective:
    \STATE \quad $\theta \leftarrow \arg \max_\theta \frac{1}{{B}} \sum_{i=1}^{{B}} \left[ \frac{1}{T} \sum_{t=1}^{T} \min\left(\frac{p_\theta}{p_{\theta_{old}}} A_t^i, \right. \right.$
\STATE \quad \quad \quad \quad $\left. \left. \text{clip}\left(\frac{p_\theta}{p_{\theta_{old}}}, 1-\epsilon, 1+\epsilon\right) A_t^i\right) \right]$
    % \STATE \quad $\theta \leftarrow \arg \max_\theta \frac{1}{B} \sum_{i=1}^{B} \frac{1}{T} \sum_{t=1}^{T} \min(\frac{p_\theta}{p_{\theta_{old}}} A_t^i, \text{clip}(\frac{p_\theta}{p_{\theta_{old}}}, 1-\epsilon, 1+\epsilon) A_t^i)$
    \STATE Update value model $V_\phi$ using L2 loss:
    \STATE \quad $L^{VF}(\phi) = \sum_{i=1}^{{B}} \sum_{t=1}^{T} \left( V_\phi(s_t^i) - V_t^i \right)^2$

    % \State \quad $L^{VF}(\phi) = \mathbb{E}_{t} \left[ (V_\phi(s_t) - V^i_t)^2 \right]$
\ENDFOR
    % \State \quad minimize $\mathbb{E}{x \sim D, y \sim \pi{\theta}(y|x)} \left[ r(\tau) - \beta \log \frac{\pi_{\theta}(y|x)}{\pi_{\text{ref}}(y|x)} \right]$
    % \State $\theta \leftarrow \theta + \alpha \nabla_\theta J(\theta)$
    % \State $\phi \leftarrow \phi + \alpha \nabla_\phi J(\phi)$
\UNTIL{maximum iteration reached}

\caption{PPO Training with Fine-grained Rewards}
\label{alg:modified_ppo_training}
\end{algorithmic}
\end{algorithm}

==> Figures/6_gpt4v_prompt.tex <==
\begin{figure*}[!h]
\centering
\includegraphics[width=\textwidth]{Figures/6_gpt4v_prompt_fig.pdf}
\caption{Prompt for GPT-4V-aided evaluation.}
\label{fig:6_gpt4v_prompt}
\end{figure*}

==> Sections/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> Tables/7_ablation_faithscore.tex <==
\begin{table*}[!t]
    \begin{center}
    \scriptsize
    \caption{Ablation of fine-grained rewards for FaithScore evaluation.}
    
    \begin{tabular}{c|c|cccccccc}
        \toprule

        \multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{7}{c}{FaithScore ($\uparrow$)} \\
        & & $\hat{f}$ & $\hat{f}_\textrm{s}$& $\hat{f}_\textrm{s,ent}$ & $\hat{f}_\textrm{s,rel}$  & $\hat{f}_\textrm{s,clr}$& $\hat{f}_\textrm{s,cnt}$ & $\hat{f}_\textrm{s,oth}$ \\
        
        \midrule
        
         \multirow{7}{*}{\textit{InstructBLIP}}
          & Baseline & 0.87 & 0.71 & 0.81 & 0.83 & 0.98 & 0.97 & 0.94  \\ \cmidrule{2-9}
          & ESREAL & \textbf{0.91} & 0.78 & 0.85 & \textbf{0.88} & 0.99 & \textbf{0.99} & 0.93 \\ \cmidrule{2-9}
          & ESREAL w/o $p_{\textrm{obj}}$ & 0.86 & 0.70 & 0.80 & 0.82 & 0.98 & 0.97 & 0.94\\
          & ESREAL w/o $p_{\textrm{att}}$ & 0.89 & 0.75 & 0.83 & 0.86 & 0.99 & 0.97 & 0.94 \\
          & ESREAL w/o $p_{\textrm{rel}}$ & 0.88 & 0.75 & 0.85 & 0.84 & 0.99 & 0.96 & 0.94 \\
          & ESREAL w/o $r_{\textrm{rec}}$ & 0.90 & \textbf{0.79} & \textbf{0.86} & 0.87 & \textbf{0.99} & 0.97 & \textbf{0.95} \\
          & ESREAL w/o $p_{\textrm{obj}}$, $p_{\textrm{att}}$, $p_{\textrm{rel}}$ & 0.80 & 0.73 & 0.83 & 0.84 & 0.98 & 0.96 & 0.95 \\
          
        \bottomrule
    \end{tabular}%
    
    \label{tab:7_ablation_faithscore}
    \end{center}
\end{table*}

==> Tables/8_rl_metrics.tex <==
\begin{table}[!h]
\caption{Reward model score evaluation results.}
\begin{center}
\scriptsize
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|ccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Method} & \multicolumn{5}{c}{RM Score ($\uparrow$)} \\
& & $p_{\textrm{obj}}$ & $p_{\textrm{att}}$  & $p_{\textrm{rel}}$  & $r_{\textrm{rec}}$  & $r_{\textrm{total}}$ \\
\midrule

\multirow{2}{*}{\textit{LLaVA}}
& Baseline & -0.68 & -0.89 & -0.09 & 0.82 & 1.62 \\
& ESREAL & \textbf{-0.44} & \textbf{-0.76} & \textbf{-0.03} & \textbf{0.83} & \textbf{2.10} \\

\midrule

\multirow{2}{*}{\textit{InstructBLIP}}
& Baseline & -0.73 & -0.78 & -0.04 & \textbf{0.83} & 1.76 \\
& ESREAL & \textbf{-0.35} & \textbf{-0.66} & \textbf{-0.01} & \textbf{0.83} & \textbf{2.28} \\

\midrule

\multirow{2}{*}{\textit{mPLUG-Owl2}}
& Baseline & -1.51 & -1.44 & -0.12 & \textbf{0.84} & 0.29 \\
& ESREAL & \textbf{-0.73} & \textbf{-0.91} & \textbf{-0.09} & 0.83 & \textbf{1.58} \\

\bottomrule
\end{tabular}%
% }
\label{tab:8_rl_metrics}
\end{center}
\end{table}
